Empirical Evaluation of Mutation-based Test Prioritization Techniques

We propose a new test case prioritization technique that combines both mutation-based and diversity-based approaches. Our diversity-aware mutation-based technique relies on the notion of mutant distinguishment, which aims to distinguish one mutant's behavior from another, rather than from the original program. We empirically investigate the relative cost and effectiveness of the mutation-based prioritization techniques (i.e., using both the traditional mutant kill and the proposed mutant distinguishment) with 352 real faults and 553,477 developer-written test cases. The empirical evaluation considers both the traditional and the diversity-aware mutation criteria in various settings: single-objective greedy, hybrid, and multi-objective optimization. The results show that there is no single dominant technique across all the studied faults. To this end, \rev{we we show when and the reason why each one of the mutation-based prioritization criteria performs poorly, using a graphical model called Mutant Distinguishment Graph (MDG) that demonstrates the distribution of the fault detecting test cases with respect to mutant kills and distinguishment.

==> discussion.tex <==
%!TEX root = stvr17.tex
\section{Discussion}
\subsection{Universally Indistinguishable Mutants}\label{sec:indistinguishable}
In mutation testing, it may be the case that a mutant and an original program are syntactically different but semantically equivalent, so that there is no test to kill the mutant. In other words, there is a mutant $m_e\in M$ generated from an original program $p_o$ such that 
\begin{equation}\label{eq:equivalent}
\forall t\in T, d(t,p_o,m_e) = 0.
\end{equation}
The mutant $m_e$ is called \textit{equivalent}. Unfortunately, deciding whether a mutant is equivalent or not is undecidable~\cite{budd1982two}. However, many researchers have attempt to tackle this problem with practical approximation \cite{madeyski2014overcoming,papadakis2015trivial,kintis2015medic}. 

In the $d$-criterion, it may be the case that two mutants are syntactically different but semantically equivalent, so that there is no test to distinguish the mutants. In other words, there are two mutants $m_x,m_y\in M'$ such that 
\begin{equation}\label{eq:indistinguishable}
\forall t\in T, d(t,p_o,m_x) = d(t,p_o,m_y)
\end{equation}
We say that $m_x$ and $m_y$ are \textit{universally indistinguishable}. Similar to the equivalent mutant detection, deciding whether two mutants are universally indistinguishable or not is clearly undecidable. Whereas attempts to solve this problem is not in the scope of this paper, we want to show how this problem is closely related to the traditional equivalent mutant detection problem. 

Intuitively, when a mutant is equivalent, it implies that the mutant and its original program are universally indistinguishable. Specifically, if we set $m_y = p_o$ in (\ref{eq:indistinguishable}), then $d(t,p_o,p_o) = 0$ for all tests so that (\ref{eq:indistinguishable}) becomes equal to (\ref{eq:equivalent}). Thus, an approach to detect the equivalent mutants is sufficient to detect the universally indistinguishable mutants. Many approaches developed to tackle the equivalent mutant detection problem are fully applicable to the universally indistinguishable mutant detection problem as well.

We should note that the notion of \textit{duplicated} mutants proposed in~\cite{papadakis2015trivial} is similar to the universally indistinguishable mutants. Two mutants are duplicated when they are not equivalent to the original program but equivalent to each other. The key difference between the notion of duplicated mutants and universally indistinguishable mutants comes from the sets of mutants they consider: the extended mutant set $M'=M\cup \{p_o\}$ is considered in universally indistinguishable mutants, whereas only the generated mutants $M$ is considered in duplicated mutants. To be precise, the set of universally indistinguishable mutants is the union of the set of duplicated mutants and the set of equivalent mutants. In other words, by adapting $M'$ instead of $M$, not only equivalent mutants but also duplicated mutants are considered together in the notion of universally indistinguishable mutants. Further attempts for solving the universally indistinguishable mutants problem will naturally solve the equivalent mutants problem and the duplicated mutants problem, together.
